Open Charm Production and its Lepton Pair Signal in High Energy Nuclear Collisions

Open charm production at the initial and the pre-equilibrium stages in nuclear collisions is studied. The pre-equilibrium contribution to open charm production in $A+A$ collisions at $\sqrt s=200 AGeV$ is shown to be very sensitive to correlations between momenta and space-time coordinates of the minijets produced after the initial collision. A minimal correlation model based on the uncertainty principle is introduced, and leads only to a small pre-equilibrium charm yield as compared with initial yields. Opposite-sign lepton pairs $ee, e\mu$ and $\mu\mu$ from open charm decay in $p+A$ reactions at $\sqrt s=200$ AGeV are proposed as a measure of nuclear shadowing effects. Via an approximate scaling, the ratio of the spectra from $p+A$ collisions to those from $pp$ collisions is shown to reflect the shadowing function well. Finally it is shown that the required measurements are feasible at RHIC.

==> abstract_f2.tex <==
{
\renewcommand{\baselinestretch}{1}
%\small

%
Open charm production at the initial and the pre-equilibrium stages in nuclear
collisions is studied.  
The pre-equilibrium contribution to open charm production in $A+A$ collisions
at $\sqrt{s}=200$AGeV is shown to be very sensitive to correlations between
momenta and space-time coordinates of the minijets produced after the initial
collision.
A minimal correlation model based on the uncertainty principle is introduced,
and leads only to a small pre-equilibrium charm yield as compared with initial
yields. 
Opposite-sign lepton pairs $ee$,$e\mu$ and $\mu\mu$ from open charm decay in
$p+A$ reactions at $\sqrt s=200$ AGeV are proposed as a measure of nuclear
shadowing effects.
Via an approximate scaling, the ratio of the spectra from $p+A$ collisions to
those from $pp$ collisions is shown to reflect the shadowing function well. 
Finally it is shown that the required measurements are feasible at RHIC. 
}


==> title_f1.tex <==
% title.tex     -       T.J. Woch       4-Jun-1988
%
% Title page and abstract for the dissertation
%
\def\bs#1{\renewcommand{\baselinestretch}{#1}}
\bs{1}
\begin{titlepage}
\vspace{0.5in}
\begin{center}
\LARGE\bf 
Open Charm Production \\
And Its Lepton Pair Signal \\
In High Energy Nuclear Collisions
\\
\vspace{1.75in}
\large
        Ziwei Lin    \\
\vspace{2.0in}
\normalsize
        Submitted in partial fulfillment of the \\
                requirements for the degree \\
                 of Doctor of Philosophy\\
        in the Graduate School of Arts and Sciences \\[.21in]
                   COLUMBIA UNIVERSITY\\
                          1996
\end{center}
\end{titlepage}

\bs{1.7}
\begin{titlepage}
\vspace{.5in}
\begin{center}
\Large\bf
                        Abstract \\
\vspace{.5in}
\large\bf
Open Charm Production And Its Lepton Pair Signal 
In High Energy Nuclear Collisions
\\
\vspace{.25in}
\rm
                Ziwei Lin    \\
\vspace{.5in}
\end{center}

\normalsize
\textwidth 370pt
\oddsidemargin 69pt             %   Left margin on odd-numbered pages.
\evensidemargin 69pt            %   Left margin on even-numbered pages.

\begin{quotation}
\noindent
\input{abstract_f2.tex}
\bs{1.7}\Huge\normalsize
\end{quotation}

\end{titlepage}
\newpage
\bs{1}\Huge\normalsize
\textwidth 390pt
\oddsidemargin 59pt             %   Left margin on odd-numbered pages.
\evensidemargin 59pt            %   Left margin on even-numbered pages.


























